The role of city geometry in determining the utility of a small urban light rail/tram system

In this work, we show the importance of considering a city's shape, as much as its population density figures, in urban transport planning. We consider in particular cities that are circular (the most common shape) compared to those that are rectangular: For the latter case we show greater utility for a single line light rail/tram system. We introduce the new concepts of Infeasible Regions and Infeasibility Factors, and show how to calculate them numerically and (in some cases) analytically. A particular case study is presented for Galway City.

==> nodes.tex <==
\node at (-0.5,0.5) { A};
\node at (-0.5,1.5) { B};
\node at (-0.5,2.5) { C};
\node at (-0.5,3.5) { D};
\node at (-0.5,4.5) { E};
\node at (-0.5,5.5) { F};
\node at (-0.5,6.5) { G};
\node at (-0.5,7.5) { H};
\node at (-0.5,8.5) { I};
%\node at (-0.5,9.5) { J};
%
\node at (0.5,9.5) { 1};
\node at (1.5,9.5) {2};
\node at (2.5,9.5) {3};
\node at (3.5,9.5) {4};
\node at (4.5,9.5) {5};
\node at (5.5,9.5) {6};
\node at (6.5,9.5) {7};
\node at (7.5,9.5) {8};
\node at (8.5,9.5) {9};
\node at (9.5,9.5) {10};
\node at (10.5,9.5) {11};
\node at (11.5,9.5) {12};
\node at (12.5,9.5) {13};
\node at (13.5,9.5) {14};
\node at (14.5,9.5) {15};
\node at (15.5,9.5) {16};
\node at (16.5,9.5) {17};
\node at (17.5,9.5) {18};
